A Semidefinite Relaxation for Sums of Heterogeneous Quadratic Forms on the Stiefel Manifold

We study the maximization of sums of heterogeneous quadratic forms over the Stiefel manifold, a nonconvex problem that arises in several modern signal processing and machine learning applications such as heteroscedastic probabilistic principal component analysis (HPPCA). In this work, we derive a novel semidefinite program (SDP) relaxation of the original problem and study a few of its theoretical properties. We prove a global optimality certificate for the original nonconvex problem via a dual certificate, which leads to a simple feasibility problem to certify global optimality of a candidate solution on the Stiefel manifold. In addition, our relaxation reduces to an assignment linear program for jointly diagonalizable problems and is therefore known to be tight in that case. We generalize this result to show that it is also tight for close-to jointly diagonalizable problems, and we show that the HPPCA problem has this characteristic. Numerical results validate our global optimality certificate and sufficient conditions for when the SDP is tight in various problem settings.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{xr-hyper}
\usepackage{hyperref}

\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

\input{packages.tex}
\input{macros.tex}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}
% \newtheorem{assumption}{Assumption}[theorem]

% Sets running headers as well as PDF title and authors
\headers{SDP for SHQF on the Stiefel}{K. Gilman, S. Burer, and L. Balzano}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{A Semidefinite Relaxation for Sums of Heterogeneous Quadratic Forms on the Stiefel Manifold\thanks{Submitted to the editors December 14, 2022.
\funding{K. Gilman and L. Balzano were supported in part by NSF CAREER award CCF-1845076, ARO YIP award W911NF1910027, AFOSR YIP award FA9550-19-1-0026, and NSF BIGDATA award IIS-1838179. L. Balzano was also supported by NSF award CCF-2331590.}}}

% Authors: full names plus addresses.
\author{Kyle Gilman\thanks{Department of Electrical and Computer Engineering, University of Michigan, Ann Arbor, MI 
  (\email{kgilman@umich.edu}).}
\and Samuel Burer\thanks{Department of Business Analytics, University of Iowa, Iowa City, IA 
  (\email{samuel-burer@uiowa.edu}).}
\and Laura Balzano\footnotemark[2]}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
